Correct Diagnosis, Better Feedback: A Symbolic-Verifier for Faithful LLM Tutoring Feedback in Logic Proofs

Effective LLM tutoring depends on correctly identifying the specific error in a student's reasoning before generating feedback. We study this problem in propositional-logic proof tutoring, where student actions can be checked against formal inference rules. We introduce a verifier-grounded architecture that separates diagnosis from language generation. Using 600 balanced student actions, we compare a zero-shot LLM detector, a fine-tuned detector, and a symbolic verifier. Each diagnosis is processed by shared rationale and feedback agents, isolating the effect of the initial diagnosis. The zero-shot detector achieves a macro-F1 of 0.191; fine-tuning raises this to 0.709 but retains systematic errors between structurally related classes. Rationales generally preserve the diagnosis supplied to them, showing that an incorrect diagnosis can be faithfully propagated through the pipeline. Feedback can likewise remain faithful to its rationale, non-revealing, and pedagogically appropriate while addressing the wrong error. Verifier-grounded feedback achieves the highest diagnostic correctness, and expert ratings largely uneven with the automatic feedback evaluations. These findings show that apparent feedback quality can conceal upstream diagnostic errors and that faithfulness must be evaluated separately from correctness. Our code is publicly available

==> sections/limitations.tex <==
B0 limittaiosn 

\paragraph{Limitations.} Our scope is antecedent-level diagnosis
within one propositional logic tutor; whether the same faithfulness
gap holds for richer error taxonomies or other symbolic domains
remains open. The result, however, does not depend on this domain: a
correct diagnosis is only as useful as its ability to survive
translation into feedback, and measuring that translation requires an
oracle, not a proxy.

we are only testing for one domain however we think it can be geenralized 
our feedback is both on mistakes and correct assessments

ethical consideration 
